QClusformer: A Quantum Transformer-based Framework for Unsupervised Visual Clustering

Unsupervised vision clustering, a cornerstone in computer vision, has been studied for decades, yielding significant outcomes across numerous vision tasks. However, these algorithms involve substantial computational demands when confronted with vast amounts of unlabeled data. Conversely, quantum computing holds promise in expediting unsupervised algorithms when handling large-scale databases. In this study, we introduce QClusformer, a pioneering Transformer-based framework leveraging quantum machines to tackle unsupervised vision clustering challenges. Specifically, we design the Transformer architecture, including the self-attention module and transformer blocks, from a quantum perspective to enable execution on quantum hardware. In addition, we present QClusformer, a variant based on the Transformer architecture, tailored for unsupervised vision clustering tasks. By integrating these elements into an end-to-end framework, QClusformer consistently outperforms previous methods running on classical computers. Empirical evaluations across diverse benchmarks, including MS-Celeb-1M and DeepFashion, underscore the superior performance of QClusformer compared to state-of-the-art methods.

==> code/PQL.tex <==
\RestyleAlgo{ruled}
\begin{algorithm}[t]
\small

\caption{Parameterized Quantum Layer}

\SetKwComment{Comment}{// }{}

\KwData{
\\$k$: number of nearest neighbors
\\$\sigma_Z$: observable
}

\Comment{Parameterized Quantum Layer}
\textbf{function} PQL($Z_i^\prime$) \textbf{do} \\
    \quad \textbf{for} h \textbf{in} range $[1, k]$ \textbf{do} \\
        \quad \quad \Comment{encode classical feature vector into quantum state}
        \quad \quad $|\psi_i^{(h)}\rangle := U(\mathbf{z}_i^{\prime(h)})$  \\
        \quad \quad \Comment{transform the quantum state}
        \quad \quad $|\psi_i^{\prime(h)}\rangle := V(\theta) |\psi_i^{(h)}\rangle$ \\
        \quad \quad \Comment{measure the quantum state}
        \quad \quad $\mathbf{z}_i^{\prime(h)} := \langle\psi_i^{\prime(h)}|\sigma_Z|\psi_i^{\prime(h)}\rangle$ \\
    \quad \textbf{done} \\
    \quad $Z_i := \{\mathbf{z}_i^{(h)}\}_{h=1}^k \in \mathbb{R}^{k \times n}$ \\
    \quad \textbf{return} $Z_i$ \\
\textbf{done}

\label{alg:PQL}
\end{algorithm}

==> code/QSA.tex <==
\RestyleAlgo{ruled}
\begin{algorithm}[t]
\small
\caption{Quantum Self-attention}

\SetKwComment{Comment}{// }{}

\KwData{
\\$k$: number of nearest neighbors
\\$\sigma_X,\sigma_Y,\sigma_Z$: observables
}

\Comment{Quantum Self-attention}
\textbf{function} QSA($Z_i$) \textbf{do} \\
    \quad \textbf{for} h \textbf{in} range $[1, k]$ \textbf{do} \\
        \quad \quad \Comment{encode classical feature vector into quantum state}
        \quad \quad $|\psi_i^{(h)}\rangle := U(\mathbf{z}_i^{(h)})$ \\
        \quad \quad \Comment{transform the quantum state}
        \quad \quad $|\psi_i^{\prime(h)}\rangle := V(\theta) |\psi_i^{(h)}\rangle$ \\
        \quad \quad \Comment{measure the quantum state}
        \quad \quad $\mathbf{q}_i^{(h)} := \langle\psi_i^{\prime(h)}|\sigma_X|\psi_i^{\prime(h)}\rangle$ \\
        \quad \quad $\mathbf{k}_i^{(h)} := \langle\psi_i^{\prime(h)}|\sigma_Y|\psi_i^{\prime(h)}\rangle$ \\
        \quad \quad $\mathbf{v}_i^{(h)} := \langle\psi_i^{\prime(h)}|\sigma_Z|\psi_i^{\prime(h)}\rangle$ \\
    \quad \textbf{done} \\
    \quad $Q_i := \{\mathbf{q}_i^{(h)}\}_{h=1}^k \in \mathbb{R}^{k \times n}$ \\
    \quad $K_i := \{\mathbf{k}_i^{(h)}\}_{h=1}^k \in \mathbb{R}^{k \times n}$ \\
    \quad $V_i := \{\mathbf{v}_i^{(h)}\}_{h=1}^k \in \mathbb{R}^{k \times n}$ \\
    \quad $Z_i^\prime := \textrm{softmax}(\frac{Q_i K_i^\top}{\sqrt{n}}) V_i \in \mathbb{R}^{k \times n}$ \\
    \quad \textbf{return} $Z_i^\prime$ \\
\textbf{done}

\label{alg:QSA}
\end{algorithm}

==> code/cluster_building.tex <==
\RestyleAlgo{ruled}
\begin{algorithm}[t]
\small
\caption{Cluster Dataset Construction}

\SetKwComment{Comment}{// }{}

\KwData{
\\$\mathcal{D} = \{x_i\}_{i=1}^N$: classical dataset
\\$\mathcal{M}$: classical feature extractor
\\$k$: number of nearest neighbors
\\$\mathcal{K}$: k-nearest neighbors algorithm
\\$W_e$: projecting weight
}

\Comment{Extract classical features}
\textbf{for} i \textbf{in} range $[1, N]$ \textbf{do} \\
    \quad$\mathbf{f}_i := \mathcal{M}(x_i)$ \\
\textbf{done} \\
$\mathcal{F} := \{\mathbf{f}_i\}_{i=1}^N \in \mathbb{R}^{k \times D}$

\Comment{Construct cluster dataset}
\textbf{for} i \textbf{in} range $[1, N]$ \textbf{do} \\
    \quad$\mathbf{c}_i := \mathbf{f}_i$ \\
    \quad$C_i := \mathcal{K}(\mathbf{c}_i, \mathcal{F}, k) \in \mathbb{R}^{k \times D}$ \\
\textbf{done} \\

\Comment{Construct sequential inputs $S_i$}
\textbf{for} i \textbf{in} range $[1, N]$ \textbf{do} \\
    \quad \textbf{for} h \textbf{in} range $[1, k]$ \textbf{do} \\
        \quad\quad$\mathbf{e}_i^{(h)} := \textrm{similarity}(\mathbf{c}_i, \mathbf{f}_i^{(h)}) \in \mathbb{R}^{k \times k}$ \\
        \quad\quad$\mathbf{s}_i^{(h)} := \mathbf{f}_i^{(h)} + \mathbf{e}_i^{(h)} W_e$ \\
    \quad \textbf{done} \\
    \quad$S_i := \{\mathbf{s}_i^{(h)}\}_{h=1}^k \in \mathbb{R}^{k \times D}$ \\
\textbf{done}
\label{alg:data_construction}
\end{algorithm}

==> tables/abl_quantum.tex <==
\begin{table}[t]
\centering
\caption{Pair-wise and BCubed evaluation with previous quantum clustering method with different numbers of classes on the DeepFashion dataset.}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|ccc|ccc}
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{100 classes}  & \multicolumn{3}{c}{Pair-wise}  & \multicolumn{3}{c}{BCubed}    \\
                              & Precision & Recall & F1-score & Precision & Recall & F1-score \\
\hline
QKMeans \cite{quiroga2021discriminating}                      & 88.06    & 81.02 & 84.40    & 89.84    & 88.00   & 88.91   \\
\textbf{QClusformer}                   & \textbf{90.37}    & \textbf{80.88} & \textbf{85.36}   & \textbf{93.99}    & \textbf{88.47} & \textbf{91.15}   \\
\hhline{=======}
\multirow{2}{*}{1000 classes} & \multicolumn{3}{c}{Pair-wise}  & \multicolumn{3}{c}{BCubed}    \\
                              & Precision & Recall & F1-score & Precision & Recall & F1-score \\
\hline
QKMeans \cite{quiroga2021discriminating}                      & 73.35    & 36.61 & 48.84   & 75.91    & 68.38 & 71.95   \\
\textbf{QClusformer}                   & \textbf{68.16}    & \textbf{45.68} & \textbf{54.70}    & \textbf{79.84}    & \textbf{70.59} & \textbf{74.93}  \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\label{tab:abl_quantum}
\end{table}

==> tables/deepfashion_ablation.tex <==
\begin{table}[t]
\centering
\caption{Pair-wise and BCubed evaluation on DeepFashion dataset with different settings: three PQCs each for query, key, and value (1Q-1K-1V); one PQC for query and key and one PQC for value (1QK-1V); and one PQC for query, key, and value (1QKV).}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|c|ccc|ccc}
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{QML} & \multirow{2}{*}{\makecell{Transformer\\Circuits}} &
\multicolumn{3}{c}{Pair-wise} & \multicolumn{3}{c}{BCubed} \\
& & \multicolumn{1}{c}{Precision} &
  \multicolumn{1}{c}{Recall} &
  \multicolumn{1}{c}{F1-score} &
  \multicolumn{1}{c}{Precision} &
  \multicolumn{1}{c}{Recall} &
  \multicolumn{1}{c}{F1-score} \\
\hline
& - & 57.35   & 25.83  & 35.62  & 79.73  & 48.89  & 60.61 \\
\cmark & 1Q-1K-1V & 41.97   & 31.08  & 35.71  & 65.57  & 55.30   & 60.00    \\
\cmark & 1QK-1V & 42.79   & 29.70   & 35.06  & 66.98  & 54.31  & 59.98 \\
\cmark & 1QKV & 43.09   & 29.67  & 35.14  & 67.55  & 54.12  & 60.10  \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\label{tab:abl_deepfashion}
\end{table}
